Z-Code++: A Pre-trained Language Model Optimized for Abstractive Summarization

This paper presents Z-Code++, a new pre-trained language model optimized for abstractive text summarization. The model extends the state of the art encoder-decoder model using three techniques. First, we use a two-phase pre-training process to improve model's performance on low-resource summarization tasks. The model is first pre-trained using text corpora for language understanding, and then is continually pre-trained on summarization corpora for grounded text generation. Second, we replace self-attention layers in the encoder with disentangled attention layers, where each word is represented using two vectors that encode its content and position, respectively. Third, we use fusion-in-encoder, a simple yet effective method of encoding long sequences in a hierarchical manner. Z-Code++ creates new state of the art on 9 out of 13 text summarization tasks across 5 languages. Our model is parameter-efficient in that it outperforms the 600x larger PaLM-540B on XSum, and the finetuned 200x larger GPT3-175B on SAMSum. In zero-shot and few-shot settings, our model substantially outperforms the competing models.

==> 1_introduction.tex <==
\section{Introduction}

 While there is a tremendous progress on pre-trained generative language foundation models recently, it still requires to train a huge generative foundation model with tens of or even hundreds of billions of parameters \citep{gpt3, chowdhery2022palm, tay2022unifying} which remains inefficient for large scale product deployment.  Z-Code\citep{wang2020multi} is proved as one of the most efficient and effective foundation model for multilingual machine translation by jointly training an encoder-decoder model with BERT-like masked language model(MLM), machine translation(MT) and denoise auto-encoder(DAE) tasks in multi-task learning way. However, text summarization, which is another central task of natural language generation(NLG), is still a challenge for current state of the art pre-training language models(PLM) as it requires the model to have a well understanding of the content and identify the important contents, then generate fluent, informative, precise and concise summary by aggregating and rewording the identified contents. Meanwhile, there is a big progress on making more efficient PLMs for natural language understanding(NLU)\citep{devlin2018bert, he2020deberta, liu2019roberta, clark2020electra, he2021debertav3, he2020deberta} tasks. For example, DeBERTaV2\textsubscript{XXLarge}\citep{he2020deberta} surpasses T5\textsubscript{11B} on SuperGLUE\citep{wang2019superglue} and GLUE\citep{wang2018glue} with less than 1/8 parameters by improving BERT-like PLMs with Disentangled Attention(DA), which is a new relative position encoding algorithm. DeBERTaV3\textsubscript{XSmall}\citep{he2021debertav3} further surpasses BERT\textsubscript{large} on a broad range of NLU tasks with only 22M parameters which is less than 1/10 of BERT\textsubscript{large} by improving ELECTRA-like PLMs with DA and Gradient Disentangled Embedding Sharing(GDES). While those techniques have shown to be effective for NLU PLMs, we are wondering if it's possible to use those techniques to improve PLMs for text summarization which requires a well understanding of the content. Along with  this direction, we propose Z-Code++, which is an extension of Z-Code by improving T5-like \citep{raffel2019t5, xue2021mt5} encoder-decoder model with DA and Replaced Token Detection (RTD)\citep{clark2020electra,he2021debertav3,meng2021coco,chi2021xlm,Kanakarajan2021SmallBenchNB} in a similar multi-task learning way as Z-Code. 
 
 Unlike PEGASUS, which uses a specifically optimized objective, Gap-Sentence-Generation(GSG), to pre-train a foundation model for text summarization, we use T5-like Corrupted Span Reconstruction(CSR). There are two folds to choose CSR instead of GSG. First, the gap sentence in GSG is selected via a ROUGE-like score, we think this will make the model more bias to ROUGE metric while hurt overall human experience. Second, CSR is more general and GSG is a special case of CSR when the randomly selected span is the same as the selected sentence in GSG. Based on the human evaluation results on XSum leaderboard, as shown in \ref{tab:xsum}, even though the improvement of ROUGE score is relatively small, the improvements on overall human score is significant, e.g. 0.49 vs 0.51. Our other experiments show that {\ModelName} outperforms PEGASUS and other state of the art generation models with similar structure and parameters on various representative text summarization tasks while remains competitive or even better performance on other NLG/NLU tasks. To the best of our knowledge, Z-Code++ is the first  language foundation model that augment a generative language model with RTD-like discriminative objective and shows substantial performance improvement on both text summarization and other NLG/NLU tasks.
 
 Specifically, we pre-train two variants of {\ModelName} models, i.e., {\ModelName}\textsubscript{large} and m{\ModelName}\textsubscript{large}. {\ModelName}\textsubscript{large} are trained with a similar way of T5\textsubscript{large} for English tasks. m{\ModelName}\textsubscript{large} is trained with a similar way as mT5\textsubscript{large} for multilingual tasks. Unlike T5, our English models are trained with 160G English data which is the same as DeBERTaV3 and use the same vocabulary as DeBERTaV2. Unlike mT5, m{\ModelName}\textsubscript{large} was trained with only 500B tokens due to lack of computation resource. 
 
 To measure the text summarizaiton performance, we evaluate them on 13 standard text summarization tasks across 5 languages. Z-Code++\textsubscript{large}/mZ-Code++\textsubscript{large} set  new state of the art numbers on 9 out of 13 text summarization tasks according to public numbers. To overcome the $O(N^2)$ memory and computation complexity to handle long document summarizaiton, we propose Fusion-in-Encoder(FiE), which is a simple but effective method inspired by Fusion-in-Decoder. With FiE, our results show \ModelName\textsubscript{large} can handle as long as 16k tokens during training and outperforms LongT5\textsubscript{xlarge} on arXiv/PubMed tasks. As the zero shot and few shot performance is critical for real-world text summarization, we first measured the 10-shot and 100-shot performance of \ModelName\textsubscript{large} on XSum, CNNDM and SAMSum, and \ModelName\textsubscript{large} outperforms PEGASUS. Inspired by T0, we further continuously train \ModelName\textsubscript{large} with multiple summarizaiton tasks with hand crafted prompts which further improves the zero shot and few shot performance. As of May, 6th, 2022, Z-Code++\textsubscript{large} sits atop of XSum leaderboard with human evaluation which surpassed UL2\textsubscript{20B}, T5\textsubscript{11B} and PEGASUS. 
 
 We also evaluate the performance of {\ModelName} models on 13 other critical NLG/NLU tasks, including WebNLG,E2E NLG, and 8 sentence classification tasks on GLUE leaderboard, XNLI, TyDiQA and SQuAD across 20 languages. 
 According to the public numbers, \ModelName\textsubscript{large}/m\ModelName\textsubscript{large} set new state of the art number on WebNLG and E2E NLG tasks. Our model remains competitive or even better on GLUE benchmark  tasks compared with models with similar model structure and parameters. Compared with current state of the art multilingual NLU models with similar model structure and parametres, m{\ModelName} outperforms mT5\textsubscript{large} and XLM-R\textsubscript{large} on XNLI and TyDiQA tasks. 
 Further more, \ModelName\textsubscript{large} outperforms PaLM\textsubscript{540B} on XSum, WebNLG-En and E2E NLG by 3.5\%, 7.0\% and 1.6\% ROUGE-2 score correspondingly, which are significant even with less than 1/600 parameters. 
  Compared with carefully fine-tuned GPT3\textsubscript{175B} with LoRA\citep{hu2021lora}, {\ModelName\textsubscript{large} } outperforms it on SAMSum which is a conversational summarization task even with less than 1/200 parameters. 
 The results makes Z-Code++ models one of the best foundation models for text summarization and a wide range of critical NLG/NLU tasks. 

==> 2_background.tex <==
\section{Background}



\subsection{Pre-training objective for text summarization}
PEGASUS is an encoder-decoder transformer\citep{vaswani2017attention}  model specifically optimized to text summarization. PEGASUS is pre-trained with Gapped Sentence Generation(GSG) objective. GSG construct pseudo summary by selecting a few sentences in the input document based on a ROUGE-like importance score which calculate the overlap of the sentence with the rest of the document. The selected sentences in the original document are replaced with a special token \textit{[MASK1]}. While GSG has been shown to effective to text summarization based on the ROUGE scores, the human evaluation score of PEGASUS on the XSum leaderboard indicate GSG pre-training is biased to automatic metric. Meanwhile, other general objective, such as Corrupted Span Prediction(CSP) and infilling are used to pre-train general text generation models, such as T5 and BART. Those models are also shown to be effective for text summarization even though the ROUGE score is not as good as PEGASUS on some tasks. CSP was first proposed in T5\citep{raffel2019t5}. T5 \cite{raffel2019t5} extends the idea of SpanBERT \cite{joshi2019spanbert}  to train an encoder-decoder model by replacing consecutive tokens with a single sentinel token and the decoder is required to reconstruct the span given the corrupted context encoding from encoder and corresponding sentinel token from decoder input. The loss function of CSP can written as, 
\begin{equation}
\label{eq:csp}
    L_{CSP} =  \mathbbm{E}\left( -\sum_{i=1}^{|\bm{Y}|}{\text{log} \;  p_{\theta}\left(\bm{Y}_i|\bm{\tilde{X}}_{CSP}, \bm{Y}_<i\right)} \right)
\end{equation}
Where $\theta$ is the parameter of encoder-decoder, $\bm{\tilde{X}}_{CSP}$ is the input with consecutive tokens replaced by a sentinel token and $\bm{Y}$ is the replaced tokens.
The experiment results of T5 on a broad range of NLU and NLG tasks shows that CSP is an effective pre-training objective for generative language models. 

Unlike T5, BART \cite{bart} was pre-trained with infilling objective which applies a similar input corruption method, while the objective is to reconstruct the whole input sentence instead of just the corrupted span. In Z-Code++ we adopt similar objective as T5, as we practically found it's more efficient than in-filling which is used for BART pre-training. 

\subsection{Replaced Token Detection}
Relaced Token Detection (RTD) was proposed in ELECTRA has shown to be an effective way to pre-train a language model for NLU tasks. ELECTRA was trained with two transformer encoders in GAN style. One is called generator trained with MLM; the other is called discriminator trained with a token-level binary classifier. The generator will replace masked tokens in the input sequence with ambiguous tokens. Then the discriminator is required to determine if a token is replaced by the generator. We use $\theta _ G$ and $\theta _ D$ to represent the parameters of the generator and the discriminator, respectively. The loss function of the generator can be written as, 
\begin{equation}
\label{eq:lg}
    L_{MLM} =  \mathbbm{E}\left( -\sum_{i\in \mathcal{C}}{\text{log} \;  p_{\theta_G}\left(\tilde{x}_{i,G}=x_i|\bm{\tilde{X}}_G\right)} \right)
\end{equation}
, where $\bm{\tilde{X}}_G$ is the input to the generator by randomly masking $15\%$ tokens in $\bm{X}$. The input sequence of the discriminator is constructed by replacing masked tokens with new tokens sampled according to the output probability from the generator:

\begin{equation}
\label{eq:xd}
\tilde{x}_{i,D} = \left\{ \begin{array}{cr}
    \tilde{x}_{i} \sim  p_{\theta_G}\left(\tilde{x}_{i,G}=x_i|\bm{\tilde{X}}_G\right),  & i \in \mathcal{C}  \\
      x_{i}, & i \notin \mathcal{C}
\end{array}\right.
\end{equation}

The loss function of the discriminator is written as,
\begin{equation}
\label{eq:ld}
    L_{RTD} =    \mathbbm{E}\left(- \sum_{i}{\text{log} \;  p_{\theta_D}\left(\mathbbm{1}\left(\tilde{x}_{i,D}=x_i\right)|\bm{\tilde{X}}_{D}, i \right)}\right)
\end{equation}

, where $\mathbbm{1}(\cdot)$ is the indicator function and $\bm{\tilde{X}}_{D}$ is the input to the discriminator constructed via \Eqref{eq:xd}. In ELECTRA, $L_{MLM}$ and $L_{RTD}$ are optimized jointly, $L = L_{MLM} + \lambda L_{RTD}$, where $\lambda$ is the weight of the discriminator loss $L_{RTD}$, which was set to 50 in ELECTRA. Z-Code++ adopts RTD to improve the efficiency of encoder-decoder model with the encoder learns a better representation of the context.

\subsection{Disentangled Attention} 
Disentangled Attention was first proposed in DeBERTa which differs from  existing approaches in that it represents each input word using two separate vectors: one for the content and the other for the position. Meanwhile, its attention weights among words are computed via disentangled matrices on both their contents and relative positions. The experiments from DeBERTa paper shows that Disentangled Attention is an efficient way to encode the positional dependency in transformer models. Z-Code++ also adopts Disentangled Attention to improve the model efficiency.

\subsection{Z-Code}
Z-Code\citep{wang2020multi} is another Transformer\citep{vaswani2017attention} based encoder-decoder model, that is proved as one of the most efficient and effective foundation model for multilingual machine translation by jointly training an encoder-decoder model with BERT-like masked language model(MLM), machine translation(MT) and denoise auto-encoder(DAE) tasks in multi-task learning way. The sharing of linguistic elements across similar languages and multi-task learning improved the quality, reduced the costs, and improved efficiency for machine translation capability in Azure Cognitive Services\footnote{\url{https://aka.ms/a-holistic-representation-toward-integrative-ai}}. While Z-Code is specifically optimized for machine translation, as an extension of Z-Code, we propose Z-Code++ which is specifically optimized for text summarization with CSP, RTD, DA and other techniques. 


==> 3_approach.tex <==
\section{Z-Code++}
\label{sec:method}
While T5-like encoder-decoder model has been shown to be effective for generative language model pre-training. Z-Code++ further improves the generation with RTD objective to enhance encoder to learn a better representation of input. The overall architecture is shown in \ref{fig:zpp}. Following BERT, for each input text sequence, we create the input of generator , $\bm{\tilde{X}_{G}}$, by replacing 15\% tokens with \texttt{[MASK]} tokens. Following T5 and BART, we create the input of encoder-decoder, $\bm{\tilde{X}}_{CSP}$, by first randomly selecting a position $k$ of $\bm{X}$ and then a random span $\bm{Y}_{k}$ from that position with an average length of $\mu$ is replaced with a sentinel token \texttt{[MASK]}$_{k}$. The process continues till the total replaced tokens reached 15\% of ${\bm{X}}$. 
%$\bm{\tilde{X}}_{CSP}$ is feed to encoder and \{ \texttt{[MASK]}$_{k}$, $\bm{Y}_{k}$ \} is feed to decoder.
The objective of CSP $L_{CSP}$ is the same as T5. Z-Code++ will be jointly optimized with $L = L_{MLM} + \left(\lambda_{RTD} L_{RTD} + \lambda_{CSP} L_{CSP} \right)$. After pre-training, only the encoder-decoder part is used for downstream task adaptation. Practically, we found $\lambda_{RTD}=30, \lambda_{CSP}=1$ works best in our setting and we apply the same parameter across all of our experiments. 
\begin{figure}[htb!]
\centering  
% \includegraphics[width=0.9\linewidth,trim={2.5cm 2.0cm 8.5cm 3.0cm},clip]{figures/Architecture_v2.pdf}

\includegraphics[width=0.9\linewidth]{figures/Architecture_v2.pdf}

\caption{Illustration of the over all pre-training architecture of Z-Code++. Z-Code++ is jointly pre-trained with RTD and CSP tasks, where we use RTD task (on the left side) to optimize the encoder and CSP (on the right side) to optimize the encoder-decoder.}

\label{fig:zpp}
\end{figure}



\subsection{Long sequence encoding}
\label{fie}
It's a challenge to encode long sequence given the $O(N^2)$ memory and computation complexity of self-attention. There are some method to alleviate the issue by applying sparse attention mechanisms. However, with sparse attention, the performance on short sequence often drops due to the loss of attention precision. Inspired by fusion-in-decoder, we propose fusion-in-encoder(FIE), a simple but effective way to encode long sequence while maintain the performance on short sequence unchanged. It works by  first splitting the input into small chunks of size $L$, e.g. 256 or 512, and applying self-attention only on those small chunks locally in the first $K$ local layers of encoder, e.g. 23, then concatenating the hidden states of those small chunks as a long sequence and apply self-attention globally among the tokens in the whole sequence via $G$, e.g. 1, fusion layers. Both the local layers and fusion layers are initialized with the corresponding weights of encoder layers of Z-Code++. If we set $L$ to be larger than the input sequence length, then it's the same as original encoder and the performance keeps the same. In our experiment, we will show that compared with LongT5 which applies sparse attention and specifically optimized for summarization, Z-Code++/FIE has competitive or even better performance on long document summarization tasks.

\subsection{Two-stage pre-training for low-resource Summarization}

The capability of being able to quickly adapt to new tasks/domains with limited training examples is vital as it is exceedingly laborious and prohibitively expensive to collect and annotate Summarization data. To enable zero/few-shot learning capability for text summarization, we employ a two stage pre-training schema \ie 1) Pre-training \ModelName{} from scratch with RTD and CSP tasks to gain the capability of text understanding and generation. 2) Grounded pre-training with instruction tuning on diverse summarization tasks to enable zero/few-shot learning. Motivated by T0~\citep{wei2021finetuned}, FLAN~\citep{sanh2022multitask}, and GODEL~\citep{GODEL}, in the grounded pre-training stage, we add diverse instructions in front of each training example as inputs to the model. For instance, a training example is represented as follows, each part is illustrated in different colors:

\begin{figure}[htb!]
\centering  
% \includegraphics[width=0.9\linewidth,trim={2.5cm 2.0cm 8.5cm 3.0cm},clip]{figures/Architecture_v2.pdf}

\includegraphics[width=0.95\linewidth]{figures/example_v2.pdf}

\caption{Examples of instructions and grounded pre-training datasets.}

\label{fig:example}
\end{figure}


% \begin{tcolorbox}[boxsep=1pt,colframe=white!90!black,colback=black!2!white]
%     \textcolor{red!70}{\ Instruction: Summarize the following news article into a one sentence summary.\\} 
%     \textcolor{brown}{Source: Officers searched properties in the Waterfront Park and Colonsay View areas of the city on Wednesday.
%     Detectives said three firearms, ammunition and a five-figure sum of money were recovered.
%     A 26-year-old man who was arrested and charged appeared at Edinburgh Sheriff Court on Thursday.\\}
%     \textcolor{blue!70}{Target: A man has appeared in court after firearms, ammunition and cash were seized by police in Edinburgh.}
% \end{tcolorbox} 
Examples of instructions and grounded pre-training datasets are listed in table~\ref{tab:grounded_pretraining}.
% --- To be removed
% Low-resource are important for low resource text summeration, as it's hard and expensive to collect supervision summerization data in real-world practice. To improve  zero-shot/few-shot text summarization, we apply a two stage pre-training schema. With the Z-Code++ pre-trained from scratch as the first stage, we further jointly train Z-Code++ model with multiple Summarizationt tasks, such as WikiHow, Newsroom, MediaSum and MultiNews. Inspired by T0 and FLAN, in the second stage, we add a diverse prompts in front of each training documents of different tasks. 
% ---
\begin{table*}[htb!]
    \centering
    \begin{adjustbox}{max width=0.95\textwidth}
    \begin{tabular}{@{\hskip1pt}l| c| l @{\hskip1pt}}
        \toprule
        Task & Genre & Instructions \\
        \midrule
        MediaSum & Interview & Summarize the following interview script into a two sentences summary. \\
            & - &  How can the following interview script be rephrased into a few sentences summary. \\ \hline
        MultiNews & News & Summarize the news article into a one sentence summary.  \\
        & - & Rephrase the news article with a few sentences.\\ \hline
        News Room & News & Summarize the news article into a one sentence summary.  \\
        & - & Rephrase the news article concisely with a few sentences.\\ \hline
        WikiHow & Wiki & Summarize the paragraph into a one sentence summary. \\
        & - & Summarize the paragraph with a few words.\\ 
        \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{
    Grounded pre-training summarization datasets and examples of instructions.
    }
    \label{tab:grounded_pretraining}
    %\vspace{-3mm}
  
\end{table*}







==> 7_ack.tex <==
%\section{Acknowledgments}
%We would like to thank Jade Huang and Nikos Karampatziakis from Microsoft Dynamics 365 AI for their proofreading the draft with a lot of valuable advice and the Microsoft Research Technology Engineering team for their help on the DGX-2 cluster. We also want to thank Yoyo Liang from Microsoft Philly team for her great support of the distributed GPU training system. 
%This effort is part of the Microsoft's AI at Scale initiative\footnote{https://innovation.microsoft.com/en-us/ai-at-scale. } and  project Alexander. We thank all that contribute to this project. 

%We also thank Davis Mueller for proofreading the paper and providing insightful comments. 
%We also thank the anonymous reviewers for valuable discussions.  
%We would also like to thanks the  Microsoft Turing project for valuable discussions and comments and Microsoft Philly team and 



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

